Large-scale Tag-based Font Retrieval with Generative Feature Learning

Font selection is one of the most important steps in a design workflow. Traditional methods rely on ordered lists which require significant domain knowledge and are often difficult to use even for trained professionals. In this paper, we address the problem of large-scale tag-based font retrieval which aims to bring semantics to the font selection process and enable people without expert knowledge to use fonts effectively. We collect a large-scale font tagging dataset of high-quality professional fonts. The dataset contains nearly 20,000 fonts, 2,000 tags, and hundreds of thousands of font-tag relations. We propose a novel generative feature learning algorithm that leverages the unique characteristics of fonts. The key idea is that font images are synthetic and can therefore be controlled by the learning algorithm. We design an integrated rendering and learning process so that the visual feature from one image can be used to reconstruct another image with different text. The resulting feature captures important font design details while is robust to nuisance factors such as text. We propose a novel attention mechanism to re-weight the visual feature for joint visual-text modeling. We combine the feature and the attention mechanism in a novel recognition-retrieval model. Experimental results show that our method significantly outperforms the state-of-the-art for the important problem of large-scale tag-based font retrieval.

==> intro-old.tex <==
\section{Introduction}\label{sec:intro}
Fonts play an important role in designing and personalizing various documents including books, posters, invitations, advertisements and digital signatures. A great number of fonts are available on different font marketplaces, such as MyFonts, Font Squirrel and Google Fonts. This burst of fonts prompts font retrieval applications. Image-based font retrieval (i.e. font recognition) is the first mature technology that has already been used on popular font websites, where a user can input an image of an unknown font and the font recognition system will return the exact or most similar fonts to the user. On the other hand, tag-based font retrieval is still an under-explored research topic. As shown in Figure~\ref{fig:intro}, it aims to retrieve the most relevant fonts from a large font pool based on user's query tags. As a complement to the existing image-based font retrieval systems, tag-based font retrieval does not require an input sample image of the desired font, which can be difficult to obtain in many cases.

The task of tag-based font retrieval is first introduced by O'Donovan et al. \cite{o2014exploratory} who collect a tag-based font dataset and train Gradient Boosted Regression Trees~\cite{friedman2001greedy} for retrieval. However, this dataset only contains 1,278 fonts annotated with 37 tags, which is very limited for user to choose from. To this end, we collect a large-scale dataset from MyFonts\footnote{https://www.myfonts.com/}, which contains images of 19,161 high-quality fonts and 1,923 unique user tags. We also employ crowd-sourcing workers to collect 1,661 tag rankings with high human consensus on a subset of fonts for evaluation purpose. This dataset will be released as a benchmark dataset for tag-based font retrieval. Based on the dataset, we investigate this problem with a deep learning framework.

\begin{figure}[!t]
\vspace{-2mm}
\centering
\includegraphics[width=3.3in]{figures/intro.pdf}
\caption{Overview of tag-based font retrieval.}
\label{fig:intro}
\vspace{-5mm}
\end{figure}



For text-based image retrieval tasks, the state-of-the-art deep learning models \cite{wang2017adversarial}\cite{reed2016learning}\cite{li2017identity}\cite{zheng2017dual} use a retrieval-based structure, which we call retrieval models. Typically, corresponding and non-corresponding image-text pairs are generated for training, and retrieval models predict a similarity score for each pair to optimize a ranking loss function.
However, as shown in Section~\ref{sec:exp}, these retrieval models perform poorly for our task because they cannot accurately embed multiple tags in different semantic levels together in the process of generating the text feature. To address this problem, we propose a combined recognition-retrieval model for this task. A tag recognition model is first trained to predict the probability of a font to match each tag. Based on the tag recognition model, a retrieval model is further trained to map the predicted tag probabilities into the final affinity score to the query. This design circumvents directly embedding multiple tags of a query together and leads to remarkable improvement. 

As the core module, our tag recognition model has a huge impact on the overall font retrieval quality. Typically, as in \cite{wang2015deepfont}, we can use different images of each font with the font's tag labels to train a convolution neural network (CNN) to  predict the tag probabilities of each image. The tag probabilities of a font can then be computed as the average of its images' tag probabilities. This approach effectively increases the training sample number. However, it also suffers from two problems.

First, the input and label are at the image level and font level, respectively. From a single input image, the model may miss much of the general style information of the corresponding font. In contrast, it may extract the features specific to individual characters of the image but not representative for the font. This will cause bias for training. 

Second, given an input font image, the model essentially extracts all its visual features (e.g. line types, thickness, smoothness) without selection, and then predicts its tag probabilities based on these visual features. However, a specific kind of feature can have different significance for the tag prediction on different font images. As shown in Figure~\ref{fig:problem}, for the upper left font image, the line type is essential in deciding its tags. Based on the ground-truth tags, this ``fancy'', ``kid'' font dramatically becomes a ``sans-serif'', ``formal'' one (lower left) when the line type changes from curved to straight. In contrast, for the upper right image, the line type has no major effect on its visual feeling. Even though its line type changes, the top tags are still ``funny'', ``informal'', ``outline'' and ``shadow''. In other words, for the upper right image, the line type feature should not have a big effect in its tag prediction. Unfortunately, vanilla recognition model cannot adaptively capture this significance change of visual features over different font images.

\begin{figure}[!t]
\centering
\includegraphics[width=3.2in]{figures/problem.pdf}
\caption{An example to illustrate that a specific kind of visual feature can have different significance for tagging on different fonts.}
\label{fig:problem}
\vspace{-5mm}
\end{figure}

To address the first problem above, we employ a generative feature learning mechanism to guide the training of the tag recognition model. Specifically, we integrate a generative adversarial sub-network to learn the mutual transform of different characters of the same font through the extracted hidden feature as a bridge. In this process, for an input image of a font, its extracted hidden features are selected to preserve more general font style information such that another image with different characters of this font can be accurately generated. In contrast, font-irrelevant information will be filtered out as noise for character transform.

For the second problem, we further design an attentive feature selection mechanism to leverage implicit attention to help the model adaptively select useful information from the hidden feature. In particular, a font classification model is trained to recognize the font class of input image. Based on the font classification result, an attention map is generated from an attention module to re-weight the hidden feature at the node level as an attentive selection process.

Our contributions are summarized as follows: 
\begin{itemize}
    \vspace{-3mm}
    \item  A large-scale font tagging dataset with a complementary high-quality evaluation set for font  research.
    \vspace{-3mm}
    \item A high-accuracy combined recognition-retrieval model designed for tag-based font retrieval.
    \vspace{-3mm}
    \item Two novel mechanisms that remarkably improve the core recognition model through effective feature learning and selection.
\end{itemize}
%During the selection stage, multiple attention maps of different glyphs are generated for each input glyph image, which reduces the errors of the attention maps.


